Driving Through Ghosts: Behavioral Cloning with False Positives

Safe autonomous driving requires robust detection of other traffic participants. However, robust does not mean perfect, and safe systems typically minimize missed detections at the expense of a higher false positive rate. This results in conservative and yet potentially dangerous behavior such as avoiding imaginary obstacles. In the context of behavioral cloning, perceptual errors at training time can lead to learning difficulties or wrong policies, as expert demonstrations might be inconsistent with the perceived world state. In this work, we propose a behavioral cloning approach that can safely leverage imperfect perception without being conservative. Our core contribution is a novel representation of perceptual uncertainty for learning to plan. We propose a new probabilistic birds-eye-view semantic grid to encode the noisy output of object perception systems. We then leverage expert demonstrations to learn an imitative driving policy using this probabilistic representation. Using the CARLA simulator, we show that our approach can safely overcome critical false positives that would otherwise lead to catastrophic failures or conservative behavior.

==> Sigma IROS Review (3)/method.tex <==
In this section, we present our behavioral cloning algorithm that can effectively leverage mediated perception even in the presence of false positives.

\subsection{Imitation Learning with Mediated Perception}

Our goal is to learn the parameters $\params$ of a policy $\pi$ that can predict robot actions $\act$ from observations $\obs$, i.e., $\pi(\obs; \params) = \act$.
%
In our case, robot actions are future way-points $\act=\{w_1, \ldots w_K\}$ passed to a downstream controller. In contrast to end-to-end sensorimotor approaches, we assume observations are not raw sensor signals but instead the outputs of a perception system (e.g., object tracks, localization and mapping information).

We estimate the policy parameters $\theta$ by behavioral cloning, i.e., by supervised learning from a set of optimal demonstrations $\{\traj_1, \ldots, \traj_n\}$ generated by an expert policy $\pi_e$. Although the expert (a.k.a.\ oracle) has access to the true world state $\state$ (e.g., ground truth position of other agents), this high-level information cannot be measured directly by the robot's sensors.
%
Therefore, we assume each demonstration $\tau_k$ consists of observation-action pairs $\tau_k = (\obs_k, \act_k)$ where observations are \textit{recorded predictions of the robot's perception system}. We, however, assume that the actions $\act$ can be accurately measured (e.g., using GNSS systems or recording CAN bus signals for cars).
%
This setup is different than standard behavioral cloning~\cite{Pomerleau1988, Schaal2003imitation, Ross2011dagger, levine2017learning, Codevilla2018, cilrs2019iccv}, as we are trying to approximate an expert while operating over a different input space:
\begin{equation}
    \pi(\obs; \params) \sim \act = \pi_e(\state)
\end{equation}
A key challenge lies in potential inconsistencies between observations $\obs$ and the true state $\state$, for instance in the presence of false positives in $\obs$. This is incompatible with supervised learning, as the same observations may yield potentially different target actions (e.g., stopping or passing through an obstacle).


\subsection{Input Uncertainty Representation via Soft BEV}
\label{sec:input_uncertainty}

To overcome inconsistencies between observations and actions, we leverage uncertainty estimates provided by modern perception systems. We model observations $\obs = (\hat{\state}, \conf)$ as pairs of estimated perceptual states $\hat{\state}$ and black-box confidence values $\conf$ in $[0; 1]$ for each state variable.
%
We assume these confidence estimates negatively correlate with error rates of the respective perception sub-systems, although they might be inaccurate. This is a reasonable assumption in practice, as there are multiple ways to achieve this, for instance via Bayesian Deep Learning~\cite{kendall17uncertainty}, ensemble methods~\cite{lakshminarayanan2017simple}, or parametric approximation~\cite{meyer2019lasernet,huang2019uncertainty}.

We do not make explicit assumptions about the distribution of $\hat{\state}$ w.r.t.\ the true state $\state$. Instead, we assume the perception system is tuned for \textit{high recall}, i.e., that all critical state variables are (noisily) captured in the estimated state. This comes at the potential expense of false positives, but corresponds to the practical setup where safety requirements are generally designed to avoid partial observability issues, as false negatives are hard to recover from.
More specifically, we tackle the inherent underlying noise in the perception system and not the issue of how to handle completely out-of-distribution cases (anomalies) in the perception system, where the confidence estimates are no longer positively linked to the true error rates.

We represent the observations $\obs$ in a birds-eye-view grid, i.e., an $N{\times}M{\times}D$-dimensional tensor $\bev$ where each dimension $k$ represents a category of estimated state (e.g., an object or feature type) together with the respective estimated confidences. Each slice $\bev_k$ is a matrix $\bev_k \in [0;1]^{N \times M}$, where each element corresponds to the presence of an estimated object or feature of type $k$ at that location, weighted by its estimated confidence.
%
\begin{comment}
From this tensor, a simple input representation that incorporates uncertainty estimates can be formulated as a sum over all binary masks, scaled by the respective confidence level of each object $i$:
\begin{equation}
    \bev_k = \sum_{i}{B_{i}*c_{i}}
\end{equation}
\end{comment}
%
We refer to the resulting input representation $\bev$ as \emph{Soft BEV}. 




\begin{figure}
\centering
\vspace*{4mm}
\includegraphics[width=0.48\textwidth]{figures/qualitative5.pdf}
\caption{Qualitative illustration of an agent using the \emph{Soft BEV} grid, successfully ignoring a false positive (top). Note that a few instances later it is able to stop for a true positive (bottom)}
\label{fig:qualitative}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Subsection 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Behavioral Cloning with Soft BEV}
\label{sec:system_setup}

We model a driving agent via a deep convolutional policy network taking as input the aforementioned Soft BEV representation $\bev$.
%
The CNN outputs way-points along the future trajectory, which are then used by a PID controller to compute the control signals for the steering and throttle of the vehicle.
%
We use the same network architecture as proposed by Codevilla \emph{et al.}~\cite{cilrs2019iccv} and Chen \emph{et al.}~\cite{chen2019learning}.
It consists of a ResNet-18~\cite{he2016deep} base network acting as an encoder, followed by three deconvolutional layers which also have as an input the current speed signal. 
For each of the potential high-level commands (``go left'', ``go right'', ``go straight'', ``follow the road''), the network predicts multiple output heat-maps which are then converted into way-points by spatial soft-argmax layers. 
%
Based on the high-level command, the respective head of the network is used to predict the way-points.

To operate correctly under uncertainty, the goal is to learn a policy that fulfills the standard behavioral cloning target, while additionally remaining invariant to the noise in the input features.
%
\begin{comment}
\begin{equation}
    \pi_{a}(\phi_t) \sim \pi_{a}(\phi_{t, noisy})
\end{equation}
\begin{equation}
    \phi_{t, noisy} = \phi_{t} + \delta_{\phi_{t}}
\end{equation}
where $\delta_{\phi_{t}}$ represents the bounded noise added to the state features. 
The agent policy is then modeled as a function of the learned policy parameters $\params$ and the feature states:
\begin{equation}
    \pi_{a}(\phi_t) = f(\phi_t; \params).
\end{equation}
\end{comment}
%
As we directly encode uncertainty in the input representation, the optimal actions (as done by the expert) can still be optimal under perceptual noise, as long as the behavioral patterns are not dominated by a wrong bias in uncertainty estimates. This is a reasonable assumption in practice, as consistent patterns of errors can be characterized on a validation set and addressed specifically. 
%
Therefore, the problem can still be treated as a supervised policy learning~\cite{Ross2011dagger,Bojarski2016nvidiadriving}, solving the following optimization problem:
\begin{equation}
    \params^* = \argmin_{\params}{\sum_{i}{l(\pi(\bev^i; \theta), \pi_{e}(\state_i))}}
    %\theta = \argmin_{\theta}{\sum_{i}{ \| (\pi_{e}(\phi_t), \pi_{a}(\phi_{t, noisy})) \|_{1} }}
\end{equation}
where $l$ is a loss function, in our case the $L_1$-distance.


\begin{comment}
The entire system is depicted in Figure~\ref{fig:system_setup}. 
At every frame the simulation provides a static BEV grid comprising of the road layout, lane lines, traffic lights, a list of dynamic objects (pedestrians and vehicles), a high-level command and additional state variables, including speed. 
The size of this BEV grid corresponds to a real-world dimension of $64m \times 64m$.

For each dynamic object we create a binary mask and scale its absolute values by the corresponding confidence score, as described in Section~\ref{sec:input_uncertainty}.
The confidence score provided by the simulation represents the uncertainty of existence for the respective object and should emulate the output uncertainty of a perception system. 
The resulting Soft BEV grid is then cropped into a reduced dimension of $38m \times 38m$ and fed into a CNN, together with the high-level command and the current speed.
The CNN outputs way-points that are then used by a PID controller to compute the control signals for the steering and throttle of the vehicle.
\end{comment}




==> Sigma IROS Review (3)/old/project_old_stuff.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% OLD Section 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\section{Representing Perceptual Uncertainty}
In this section we present our approach for modeling observations generated from a perception stack.
\begin{itemize}
    \item Introduce the BEV representation
    \begin{itemize}
        \item Dimensions of BEV, layers, etc
        \item What are the benefits of parametric BEV? Can manipulate on object level, and allows to play around with all kinds of noise models. Also it is interpretable. Additionally, other papers have shown (LBC, planer bev planner) that it is a very useful representation. 
    \end{itemize}
    \item Assumptions
    \begin{itemize}
        \item No SLAM noise. GT road layout, lane lines, traffic lights  and traffic light signal
        \item Noise on pedestrians and vehicles in the form of a FP flicker - For pedestrians it is potentially useful to add Gaussian noise.
        \item What are the benefits of parametric BEV? Can manipulate on object level, and allows to play around with all kinds of noise models. Also it is interpretable. Additionally, other papers have shown (LBC, planer bev planner) that it is a very useful representation. 
    \end{itemize}
    \item Model for TP/FP flicker
    \item Model for temporal flicker and proof that it is bounded!
    \item Explain how the uncertainty associated with the models is incorporated into the BEV representation. Explain the benefits of non-parametric representations.
    \begin{itemize}
        \item MUST INTRODUCE MULTIPLE POTENTIAL UNCERTAINTY REPRESENTATIONS: Scale in same layer, have an additional uncertainty layer, 
    \end{itemize}
\end{itemize}
\fi 

==> Sigma IROS Review (3)/tables/3ddet_metrics.tex <==
% \usepackage{colortbl}

\centering
\arrayrulecolor[rgb]{0.8,0.8,0.8}
\begin{tabular}{|l|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{3D-Detector} & \multicolumn{3}{c|}{$AP_{Car}$} & \multicolumn{3}{c|}{$AP_{Ped}$} \\ 
& 0.5m & 1.0m & 2.0m & 0.5m & 1.0m & 2.0m \\
\hline
\multicolumn{7}{|c|}{Objects closer than 25m} \\ 
\hline
PP - 32 beams & 90.7 & 92.8 & 95.8 & 58.8 & 60.6 & 61.8 \\
\hline
PP - 64 beams & 84.0 & 90.5 & 93.2 & 60.1 & 68.1 & 69.4 \\
\hline

 \multicolumn{7}{|c|}{Objects closer than 50m} \\ 
\hline
PP  - 32 beams & 65.5 & 69.6 & 74.5 & 27.4 & 28.1 & 29.0 \\
\hline
PP  - 64 beams & 62.2 & 72.6 & 75.8 & 38.9 & 44.0 & 45.22 \\
\hline

\end{tabular}
\arrayrulecolor{black}


==> Sigma IROS Review (3)/tables/experiment_schedule.tex <==
\begin{table}
\centering
\arrayrulecolor{black}
\begin{tabular}{!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}} 
\hline
\multicolumn{1}{!{\color[rgb]{0.8,0.8,0.8}\vrule}l!{\color{black}\vrule}}{} & \multicolumn{1}{c!{\color{black}\vrule}}{TRAINING} & \multicolumn{4}{c!{\color{black}\vrule}}{TESTING}                                                                                                       \\ 
\hline
Model                                                                       & Noise config                                       & \begin{tabular}[c]{@{}l@{}}FP \\noise\end{tabular} & Threshold & Bernoulli    & Bias                                                                    \\ 
\hline
BEV 1                                                                       & Noise-free                                         & no                                                 & n/a       & n/a          & n/a                                                                     \\ 
\hline
BEV 1                                                                       & Noise-free                                         & yes                                                & no        & low (0.1)    & no                                                                      \\ 
\hline
BEV 1                                                                       & Noise-free                                         & yes                                                & yes       & low (0.1)    & no                                                                      \\ 
\hline
BEV 2                                                                       & FP, unbiased                                       & yes                                                & no        & low (0.1)    & no                                                                      \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & yes       & low (0.1)    & no                                                                      \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & low (0.1)    & no                                                                      \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & medium (0.3) & no                                                                      \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & high (0.5)   & no                                                                      \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & low (0.1)    & \begin{tabular}[c]{@{}l@{}}low (mu 0.01, \\sigma 0.005)\end{tabular}    \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & low (0.1)    & \begin{tabular}[c]{@{}l@{}}medium (mu 0.05, \\sigma 0.01)\end{tabular}  \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & low (0.1)    & \begin{tabular}[c]{@{}l@{}}high (mu 0.1, \\sigma 0.02)\end{tabular}     \\
\hline
\end{tabular}
\arrayrulecolor{black}
\end{table}

==> Sigma IROS Review (3)/tables/result_3ddetector.tex <==
% \usepackage{colortbl}

\centering
\arrayrulecolor[rgb]{0.8,0.8,0.8}
\begin{tabular}{|l|c|c|} 
\hline
                                                       & \multicolumn{2}{c|}{Collision Rates}                                                                                                                                                                                                 \\ 
\hline
\multicolumn{1}{|c!{\color{black}\vrule}}{3D-Detector} & \multicolumn{1}{l!{\color{black}\vrule}}{\begin{tabular}[c]{@{}l@{}}BEV Agent with \\0.5-Threshold\end{tabular}} & \multicolumn{1}{c!{\color{black}\vrule}}{\begin{tabular}[c]{@{}c@{}}Soft BEV Agent, \\no Threshold\end{tabular}}  \\ 
\arrayrulecolor{black}\hline
PP - 32 beams                                     & 10\%                                                                                                             & 5\%                                                                                                               \\ 
\arrayrulecolor[rgb]{0.8,0.8,0.8}\hline
PP - 64 beams                                     & 5\%                                                                                                              & 5\%                                                                                                               \\
\hline
\end{tabular}
\arrayrulecolor{black}


==> Sigma IROS Review (3)/tables/result_bias.tex <==
\centering
\arrayrulecolor[rgb]{0.8,0.8,0.8}
\begin{tabular}{|l|c|c|c|c|c|} 
\arrayrulecolor{black}\hline
\multicolumn{1}{|l!{\color{black}\vrule}}{Model} & \multicolumn{1}{c!{\color{black}\vrule}}{Noise Injection} & \multicolumn{1}{c!{\color{black}\vrule}}{3-Sigma Threshold} & \multicolumn{1}{c!{\color{black}\vrule}}{p-existence} & \multicolumn{1}{c!{\color{black}\vrule}}{Bias [Mu, Sigma]} & \multicolumn{1}{c!{\color{black}\vrule}}{Benchmark Success Rate}  \\ 
\hline
Soft BEV Agent                                   & \checkmark                                                         & x                                                           & Low, 0.05                                             & x                                                          & 97.5\%                                                            \\ 
\arrayrulecolor[rgb]{0.8,0.8,0.8}\hline
Soft BEV Agent                                   & \checkmark                                                         & x                                                           & Medium, 0.1                                           & x                                                          & 92.5\%                                                            \\ 
\hline
Soft BEV Agent                                   & \checkmark                                                         & x                                                           & High, 0.5                                             & x                                                          & 95.0\%                                                            \\ 
\hline
Soft BEV Agent                                   & \checkmark                                                         & x                                                           & Low, 0.05                                             & Low, [0.01, 0.005]                                         & 92.5\%                                                            \\ 
\hline
Soft BEV Agent                                   & \checkmark                                                         & x                                                           & Low, 0.05                                             & Medium, [0.05, 0.025]                                      & 90.0\%                                                            \\ 
\hline
Soft BEV Agent                                   & \checkmark                                                         & x                                                           & Low, 0.05                                             & High, [0.2, 0.1]                                           & 92.5\%                                                            \\
\hline
\end{tabular}
\arrayrulecolor{black}


==> Sigma IROS Review (3)/tables/result_summary.tex <==
% \usepackage{colortbl}


\centering
\arrayrulecolor[rgb]{0.8,0.8,0.8}
\begin{tabular}{|c|l|c|c|c|c|c|c|c|c|} 
\arrayrulecolor{black}\hline
\multicolumn{1}{|c!{\color{black}\vrule}}{Config.} & \multicolumn{1}{l!{\color{black}\vrule}}{Model} & \multicolumn{1}{c!{\color{black}\vrule}}{Noise} & \multicolumn{1}{c!{\color{black}\vrule}}{3-Sigma threshold} & \multicolumn{1}{c!{\color{black}\vrule}}{p-existence} & \multicolumn{1}{c!{\color{black}\vrule}}{Bias [Mu, Sigma]} & \multicolumn{1}{c!{\color{black}\vrule}}{Speed} & \multicolumn{1}{c!{\color{black}\vrule}}{Acceleration} & \multicolumn{1}{c!{\color{black}\vrule}}{Jerk} & \multicolumn{1}{c!{\color{black}\vrule}}{Collision}  \\ 
\hline
1                                                  & BEV Agent                                       & x                                               & Not applicable                                              & Not applicable                                        & Not applicable                                             & 4.2                                             & 2.5                                                    & 20.5                                           & 0\%                                                  \\ 
\arrayrulecolor[rgb]{0.8,0.8,0.8}\hline
2                                                  & BEV Agent                                       & \checkmark                                               & x                                                           & Low, 0.1                                              & x                                                          & 3.2                                             & 2.8                                                    & 24.1                                           & 0\%                                                  \\ 
\hline
3                                                  & BEV Agent                                       & \checkmark                                               & \checkmark                                                           & Low, 0.1                                              & x                                                          & 4.0                                             & 2.5                                                    & 20.6                                           & 5\%                                                  \\ 
\hline
4                                                  & BEV Agent                                       & \checkmark                                               & \checkmark                                                           & Low, 0.1                                              & High, [0.2, 0.1]                                           & 3.9                                             & 2.5                                                    & 21.0                                           & 5\%                                                  \\ 
\hline
5                                                  & Soft BEV Agent                                  & \checkmark                                               & x                                                           & Low, 0.1                                              & x                                                          & 4.2                                             & 2.5                                                    & 20.4                                           & 5\%                                                  \\ 
\hline
6                                                  & Soft BEV Agent                                  & \checkmark                                               & x                                                           & Low, 0.1                                              & High, [0.2, 0.1]                                           & 4.2                                             & 2.5                                                    & 20.3                                           & 5\%                                                  \\
\hline
\end{tabular}
\arrayrulecolor{black}


==> Sigma IROS Review (3)/tables/results.tex <==
% \usepackage{colortbl}

\begin{tabular}{|l|c|c|c|c|c|c|} 
\hline
MOCK TABLE                                       & \multicolumn{4}{c|}{Noise Setup when Testing}                                                                                                                                                                                                & \multicolumn{2}{c|}{T-Test Results}                                                                        \\ 
\hline
\multicolumn{1}{|l!{\color{black}\vrule}}{Model} & \multicolumn{1}{c!{\color{black}\vrule}}{Noise Injection} & \multicolumn{1}{c!{\color{black}\vrule}}{3-Sigma Threshold} & \multicolumn{1}{c!{\color{black}\vrule}}{p-existence} & \multicolumn{1}{c!{\color{black}\vrule}}{Bias [Mu, Sigma]} & \multicolumn{1}{c!{\color{black}\vrule}}{t-statistic} & \multicolumn{1}{c!{\color{black}\vrule}}{p-value}  \\ 
\arrayrulecolor{black}\hline
BEV Agent                                        & No                                                        & Not applicable                                              & Not applicable                                        & Not applicable                                             & 0                                                     & 1                                                  \\ 
\arrayrulecolor[rgb]{0.8,0.8,0.8}\hline
BEV Agent                                        & ✓                                                         & x                                                           & Low, 0.05                                             & x                                                          & -1.5                                                  & 0.01                                               \\ 
\hline
BEV Agent                                        & ✓                                                         & ✓                                                           & Low, 0.05                                             & x                                                          & -1                                                    & 0.02                                               \\ 
\hline
Soft BEV Agent                                   & ✓                                                         & x                                                           & Low, 0.05                                             & x                                                          & -0.1                                                  & 0.5                                                \\ 
\hline
Soft BEV Agent                                   & ✓                                                         & x                                                           & Medium, 0.1                                           & x                                                          & -0.2                                                  & 0.4                                                \\ 
\hline
Soft BEV Agent                                   & ✓                                                         & x                                                           & High, 0.5                                             & x                                                          & -0.3                                                  & 0.3                                                \\ 
\hline
Soft BEV Agent                                   & ✓                                                         & x                                                           & Low, 0.1                                              & Low, [0.01, 0.005]                                         & -0.1                                                  & 0.5                                                \\ 
\hline
Soft BEV Agent                                   & ✓                                                         & x                                                           & Low, 0.1                                              & Medium, [0.01, 0.005]                                      & -1                                                    & 0.02                                               \\ 
\hline
Soft BEV Agent                                   & \checkmark                                                         & x                                                           & Low, 0.1                                              & High, [0.01, 0.005]                                        & -2                                                    & 0.01                                               \\
\hline
\end{tabular}


==> old/project_old_stuff.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% OLD Section 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\section{Representing Perceptual Uncertainty}
In this section we present our approach for modeling observations generated from a perception stack.
\begin{itemize}
    \item Introduce the BEV representation
    \begin{itemize}
        \item Dimensions of BEV, layers, etc
        \item What are the benefits of parametric BEV? Can manipulate on object level, and allows to play around with all kinds of noise models. Also it is interpretable. Additionally, other papers have shown (LBC, planer bev planner) that it is a very useful representation. 
    \end{itemize}
    \item Assumptions
    \begin{itemize}
        \item No SLAM noise. GT road layout, lane lines, traffic lights  and traffic light signal
        \item Noise on pedestrians and vehicles in the form of a FP flicker - For pedestrians it is potentially useful to add Gaussian noise.
        \item What are the benefits of parametric BEV? Can manipulate on object level, and allows to play around with all kinds of noise models. Also it is interpretable. Additionally, other papers have shown (LBC, planer bev planner) that it is a very useful representation. 
    \end{itemize}
    \item Model for TP/FP flicker
    \item Model for temporal flicker and proof that it is bounded!
    \item Explain how the uncertainty associated with the models is incorporated into the BEV representation. Explain the benefits of non-parametric representations.
    \begin{itemize}
        \item MUST INTRODUCE MULTIPLE POTENTIAL UNCERTAINTY REPRESENTATIONS: Scale in same layer, have an additional uncertainty layer, 
    \end{itemize}
\end{itemize}
\fi 

==> tables/experiment_schedule.tex <==
\begin{table}
\centering
\arrayrulecolor{black}
\begin{tabular}{!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}} 
\hline
\multicolumn{1}{!{\color[rgb]{0.8,0.8,0.8}\vrule}l!{\color{black}\vrule}}{} & \multicolumn{1}{c!{\color{black}\vrule}}{TRAINING} & \multicolumn{4}{c!{\color{black}\vrule}}{TESTING}                                                                                                       \\ 
\hline
Model                                                                       & Noise config                                       & \begin{tabular}[c]{@{}l@{}}FP \\noise\end{tabular} & Threshold & Bernoulli    & Bias                                                                    \\ 
\hline
BEV 1                                                                       & Noise-free                                         & no                                                 & n/a       & n/a          & n/a                                                                     \\ 
\hline
BEV 1                                                                       & Noise-free                                         & yes                                                & no        & low (0.1)    & no                                                                      \\ 
\hline
BEV 1                                                                       & Noise-free                                         & yes                                                & yes       & low (0.1)    & no                                                                      \\ 
\hline
BEV 2                                                                       & FP, unbiased                                       & yes                                                & no        & low (0.1)    & no                                                                      \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & yes       & low (0.1)    & no                                                                      \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & low (0.1)    & no                                                                      \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & medium (0.3) & no                                                                      \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & high (0.5)   & no                                                                      \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & low (0.1)    & \begin{tabular}[c]{@{}l@{}}low (mu 0.01, \\sigma 0.005)\end{tabular}    \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & low (0.1)    & \begin{tabular}[c]{@{}l@{}}medium (mu 0.05, \\sigma 0.01)\end{tabular}  \\ 
\hline
Soft BEV                                                                    & FP, unbiased                                       & yes                                                & no        & low (0.1)    & \begin{tabular}[c]{@{}l@{}}high (mu 0.1, \\sigma 0.02)\end{tabular}     \\
\hline
\end{tabular}
\arrayrulecolor{black}
\end{table}

==> tables/results.tex <==
% \usepackage{colortbl}

\begin{tabular}{|l|c|c|c|c|c|c|} 
\hline
MOCK TABLE                                       & \multicolumn{4}{c|}{Noise Setup when Testing}                                                                                                                                                                                                & \multicolumn{2}{c|}{T-Test Results}                                                                        \\ 
\hline
\multicolumn{1}{|l!{\color{black}\vrule}}{Model} & \multicolumn{1}{c!{\color{black}\vrule}}{Noise Injection} & \multicolumn{1}{c!{\color{black}\vrule}}{3-Sigma Threshold} & \multicolumn{1}{c!{\color{black}\vrule}}{p-existence} & \multicolumn{1}{c!{\color{black}\vrule}}{Bias [Mu, Sigma]} & \multicolumn{1}{c!{\color{black}\vrule}}{t-statistic} & \multicolumn{1}{c!{\color{black}\vrule}}{p-value}  \\ 
\arrayrulecolor{black}\hline
BEV Agent                                        & No                                                        & Not applicable                                              & Not applicable                                        & Not applicable                                             & 0                                                     & 1                                                  \\ 
\arrayrulecolor[rgb]{0.8,0.8,0.8}\hline
BEV Agent                                        & ✓                                                         & x                                                           & Low, 0.05                                             & x                                                          & -1.5                                                  & 0.01                                               \\ 
\hline
BEV Agent                                        & ✓                                                         & ✓                                                           & Low, 0.05                                             & x                                                          & -1                                                    & 0.02                                               \\ 
\hline
Soft BEV Agent                                   & ✓                                                         & x                                                           & Low, 0.05                                             & x                                                          & -0.1                                                  & 0.5                                                \\ 
\hline
Soft BEV Agent                                   & ✓                                                         & x                                                           & Medium, 0.1                                           & x                                                          & -0.2                                                  & 0.4                                                \\ 
\hline
Soft BEV Agent                                   & ✓                                                         & x                                                           & High, 0.5                                             & x                                                          & -0.3                                                  & 0.3                                                \\ 
\hline
Soft BEV Agent                                   & ✓                                                         & x                                                           & Low, 0.1                                              & Low, [0.01, 0.005]                                         & -0.1                                                  & 0.5                                                \\ 
\hline
Soft BEV Agent                                   & ✓                                                         & x                                                           & Low, 0.1                                              & Medium, [0.01, 0.005]                                      & -1                                                    & 0.02                                               \\ 
\hline
Soft BEV Agent                                   & \checkmark                                                         & x                                                           & Low, 0.1                                              & High, [0.01, 0.005]                                        & -2                                                    & 0.01                                               \\
\hline
\end{tabular}

